Online Similarity Prediction of Networked Data from Known and Unknown Graphs

We consider online similarity prediction problems over networked data. We begin by relating this task to the more standard class prediction problem, showing that, given an arbitrary algorithm for class prediction, we can construct an algorithm for similarity prediction with "nearly" the same mistake bound, and vice versa. After noticing that this general construction is computationally infeasible, we target our study to {\em feasible} similarity prediction algorithms on networked data. We initially assume that the network structure is {\em known} to the learner. Here we observe that Matrix Winnow \cite{w07} has a near-optimal mistake guarantee, at the price of cubic prediction time per round. This motivates our effort for an efficient implementation of a Perceptron algorithm with a weaker mistake guarantee but with only poly-logarithmic prediction time. Our focus then turns to the challenging case of networks whose structure is initially {\em unknown} to the learner. In this novel setting, where the network structure is only incrementally revealed, we obtain a mistake-bounded algorithm with a quadratic prediction time per round.

==> bibliography1.tex <==


\begin{thebibliography}{99} 

\bibitem{AAKKLT08}
N.~Alon, C.~Avin, M.~Kouck\'{y}, G.~Kozma, Z.~Lotker, and M.R. Tuttle.
\newblock Many random walks are faster than one.
\newblock In \emph{Proc. of the 20th Annual ACM Symposium on Parallel
  Algorithms and Architectures}, pages 119--128. Springer, 2008.

\bibitem{Bro89}
A.~Broder.
\newblock Generating random spanning trees.
\newblock In \emph{Proc. of the 30th Annual Symposium on Foundations of
  Computer Science}, pages 442--447. IEEE Press, 1989.

\bibitem{ccg10}
G. Cavallanti, N. Cesa-Bianchi, and C. Gentile. 
Linear algorithms for online multitask classification.
{\em Journal of Machine Learning Research}, 11, pp. 2901--2934, 2010. 

\bibitem{CGV09b}
N.~Cesa-Bianchi, C.~Gentile, and F.~Vitale.
\newblock Fast and optimal prediction of a labeled tree.
\newblock In \emph{Proceedings of the 22nd Annual Conference on Learning
  Theory}. Omnipress, 2009.

\bibitem{CGVZ10}
N.~Cesa-Bianchi, C.~Gentile, F.~Vitale, and G. Zappella.
\newblock Random spanning trees and the prediction of weighted graphs.
\newblock In \emph{Proceedings of the 27th International Conference on Machine Learning (27th ICML)}, 2010.

\bibitem{CGVZ10b}
N.~Cesa-Bianchi, C.~Gentile, F.~Vitale, and G. Zappella.
Active learning on trees and graphs.
In {\em Proceedings of the 23rd Conference on Learning Theory (23rd COLT)}, 2010. 

\bibitem{clr90}
T.H. Cormen, C.E. Leiserson, and R.L. Rivest.
{\em Introduction to algorithms}, MIT Press, 1990.

\bibitem{gy03}
J. L. Gross and J. Yellen (Eds.) Handbook of graph theory.
CRC Press, 2003.

\bibitem{g03}
C. Gentile.
The robustness of the $p$-norm algorithms.
{\em  Machine Learning}, 53/3 (2003), pp. 265--299. 

\bibitem{gls97}
A. J. Grove, N. Littlestone and D. Schuurmans.
General convergence results for linear discriminant updates.
{\em  Machine Learning}, 43/3 (2001), pp. 173--210.

\bibitem{Her08}
M.~Herbster.
\newblock Exploiting cluster-structure to predict the labeling of a graph.
\newblock In \emph{Proc. of the 19th International Conference on
  Algorithmic Learning Theory}, pages 54--69. Springer, 2008.

\bibitem{HL09}
M.~Herbster and G.~Lever.
\newblock Predicting the labelling of a graph via minimum $p$-seminorm
  interpolation.
\newblock In \emph{Proc. of the 22nd Annual Conference on Learning
  Theory}. Omnipress, 2009.

\bibitem{HP07}
M.~Herbster and M.~Pontil.
\newblock Prediction on a graph with the {P}erceptron.
\newblock In \emph{Advances in Neural Information Processing Systems 21}, pages
  577--584. MIT Press, 2007.

\bibitem{HPW05}
M.~Herbster, M.~Pontil, and L.~Wainer.
\newblock Online learning over graphs.
\newblock In \emph{Proc. of the 22nd International Conference on Machine
  Learning}, pages 305--312. ACM Press, 2005.

\bibitem{HLP09}
M.~Herbster, G.~Lever, and M.~Pontil.
\newblock Online prediction on large diameter graphs.
\newblock In \emph{Advances in Neural Information Processing Systems 22}, pages 649--656. 
MIT Press, 2009.

\bibitem{HPR09}
M.~Herbster, M.~Pontil, and S.~Rojas-Galeano.
\newblock Fast prediction on a tree.
\newblock In \emph{Advances in Neural Information Processing Systems 22}, pages 657--664.
MIT Press, 2009.

\bibitem{kst12}
S. M. Kakade, S. Shalev-Shwartz, A. Tewari.
Regularization Techniques for Learning with Matrices.
{\em Journal of Machine Learning Research}, 13, pp. 1865--1890, 2012. 

\bibitem{litt88}
Littlestone, N.
Learning quickly when irrelevant attributes abound: 
A new linear-threshold algorithm.
{\em Machine Learning}, 2, 285--318, 1988.

\bibitem{lp10}
R.~Lyons and Y.~Peres.
\newblock Probability on trees and networks.
\newblock Manuscript, 2010.

\bibitem{w07}
M. Warmuth. Winnowing Subspaces. ICML 2007.

\bibitem{Wil96}
D.B. Wilson.
\newblock Generating random spanning trees more quickly than the cover time.
\newblock In \emph{Proc. of the 28th ACM Symposium on the Theory of
  Computing}, pages 296--303. ACM Press, 1996.

\end{thebibliography}




==> conclusions1.tex <==
% !TEX root = main7.tex

\vspace{-0.1in}
\section{Conclusions and work in progress}
\vspace{-0.05in}
%
- any problem to lift it to weighted graphs ?

- improve bound for unknown graph case with other regularization
  technique ? (quartic dependence --> quadratic dependence without
  adding extra linear factors like O(n))

- randomize the algorithm in sect. 5 ?


